FineREX: Fine-Tuned NER-RE for Human Smuggling Knowledge Graphs

Court proceedings contain valuable evidence about human smuggling networks, but this information is often buried within unstructured, jargon-heavy legal documents. While large language models (LLMs) can support knowledge graph construction through automated information extraction, existing approaches rely on general-purpose models that are not tailored to the entity and relationship definitions required in this domain. We introduce FineREX, a streamlined knowledge graph construction pipeline built around a fine-tuned LLM for named entity recognition and relationship extraction (NER-RE). Using a manually annotated dataset of $512$ text chunks, FineREX achieves absolute improvements of 15.50% and 31.46% in entity and relationship F1-score, respectively, compared to a larger general-purpose baseline. These gains translate into higher-quality knowledge graphs, reducing legal noise by nearly half and lowering node duplication on long documents from 17.78% to 11.17%. By eliminating document rewriting and redundant extraction stages, FineREX also reduces end-to-end processing time by 50.0%. Our results demonstrate that domain-specific fine-tuning can substantially outperform larger general-purpose models while improving both the quality and efficiency of knowledge graph construction for illicit network analysis.

==> dataset.tex <==
\begin{table}[h]
\centering
\caption{Entity type distribution in the annotated dataset}
\begin{tabular}{lrr}
\toprule
\textbf{Entity Type} & \textbf{Count} & \textbf{\%} \\
\midrule
Person                   & 895 & 45.6 \\
Location                 & 567 & 28.9 \\
Means of Transportation  & 284 & 14.5 \\
Organization             & 116 &  5.9 \\
Routes                   &  71 &  3.6 \\
Smuggled Items           &  18 &  0.9 \\
Means of Communication   &  11 &  0.6 \\
\midrule
\textbf{Total}           & 1962 & 100.0 \\
\bottomrule
\end{tabular}
\label{tab:entity-dist}
\end{table}
